Prediction under Latent Subgroup Shifts with High-Dimensional Observations

We introduce a new approach to prediction in graphical models with latent-shift adaptation, i.e., where source and target environments differ in the distribution of an unobserved confounding latent variable. Previous work has shown that as long as "concept" and "proxy" variables with appropriate dependence are observed in the source environment, the latent-associated distributional changes can be identified, and target predictions adapted accurately. However, practical estimation methods do not scale well when the observations are complex and high-dimensional, even if the confounding latent is categorical. Here we build upon a recently proposed probabilistic unsupervised learning framework, the recognition-parametrised model (RPM), to recover low-dimensional, discrete latents from image observations. Applied to the problem of latent shifts, our novel form of RPM identifies causal latent structure in the source environment, and adapts properly to predict in the target. We demonstrate results in settings where predictor and proxy are high-dimensional images, a context to which previous methods fail to scale.

==> graphical_models/graphical_model.tex <==
\definegmnode{X}(-2,+0) {graphmod obs, node var={X}}
\definegmnode{W}(+2,+0) {graphmod obs, node var={W}}
\definegmnode{U} (+0,+0) {graphmod lat, node var={U}}
\definegmnode{C} (-1,-2) {graphmod obs, node var={C}}
\definegmnode{Y} (1,-2) {graphmod obs, node var={Y}}



%\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmdefaultnodes{X,W,U,C,Y}


\definegmgraph[genconf][1][]{\defaultnodes[#1]
  \dedges[#1]{{U}{W},{U}{X},{U}{C},{U}{Y},{C}{Y},{X}{C}}
  }
  
 



==> m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Option to tikzpicture to set coords based on column/text size
\def\c@@rdx(#1,#2){#1}
\def\c@@rdy(#1,#2){#2}
\tikzset{%
  fit to column/.style={x ={($\c@@rdx#1*(\columnwidth,0)$)},y={($\c@@rdy#1*(0,\textheight)$)}},
  fit to column/.default={(1,1)}
}

%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecated

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> m.symbols.tex <==
\RequirePackage{ifthen}

% use | for math mode
%\catcode`\|=3


%% Misc useful symbols

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% conditional independence
\newcommand{\cind}{{\bot\negthickspace\negthickspace\bot}} 
\newcommand{\notcind}{{\smash{\kern0.1em\not\kern-.1em}\cind}}

% fractions
% 
%% \newcommand{\bfrac}{\mathchoice{%
%%     {
%% \newcommand{\sfrac}
% this is a slightly tighter version of \frac, but in the current mathstyle (unlike \tfrac etc.).  
\newcommand{\tightfrac}[3][0.5]{\mathchoice%
    {\frac{\raisebox{-#1ex}{$\textstyle #2$}}{\raisebox{#1ex}{$\textstyle #3$}}}%
    {\frac{\raisebox{-#1ex}{$\scriptstyle #2$}}{\raisebox{#1ex}{$\scriptstyle #3$}}}%
    {\frac{\raisebox{-#1ex}{$\scriptscriptstyle #2$}}{\raisebox{#1ex}{$\scriptscriptstyle #3$}}}%
    {\frac{\raisebox{-#1ex}{$\scriptscriptstyle #2$}}{\raisebox{#1ex}{$\scriptscriptstyle #3$}}}%
}
\newcommand{\half}{\ensuremath{\tightfrac{1}{2}}}
\newcommand{\thalf}{\ensuremath{\tfrac12}}
\newcommand{\overN}{\ensuremath{\tfrac{1}{N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}




%% Utilities to define pretty functions
\makeatletter

% Functions with resizeable delimiters
%
% \DeclareResizableDelimFunction{macroname}{symbol}{left delim}{right delim}
%
% E.g. \DeclareResizableDelimFunction{foo}{\text{foo}}[]
% defines:
% \foo{x} -> \text{foo} \left[ x \right]
% \foo[\big]{x} -> \text{foo} \big[ x \big]
\def\DeclareResizableDelimFunction#1#2#3#4{
  \expandafter\newcommand\csname#1\endcsname[2][]{%
    #2\lr[##1]#3#4{##2}}}

% \DeclareResizableDelimFunction{macroname}{symbol}{left delim}{right delim}{separator}
%
% E.g. \DeclareResizableDelimFunction{foo}{\text{foo}}[]{,}
% defines:
% \foo{x}{y} -> \text{foo} \left[ x , y\right]
% \foo[\big]{x}{y} -> \text{foo} \big[ x , y \big]
%
% \DeclareResizableDelimFunction{foo}{\text{foo}}[]{\lrmid \|}
% defines:
% \foo{x}{y} -> \text{foo} \left[ x \middle \|  y\right]
% \foo[\big]{x}{y} -> \text{foo} \big[ x \big \|  y \big]
\def\DeclareResizableDelimFunctionOnTwoArgs#1#2#3#4#5{
  \expandafter\newcommand\csname#1\endcsname[3][]{%
    #2\lr[##1]#3#4{##2 #5 ##3}}}

% Optional subscripted functions with resizeable delimiters
%
% \DeclareOptSubscriptedFunction{macroname}{symbol}[default subscr]{left delim}{right delim}
%
% E.g. \DeclareOptSubscriptedFunction{foosq}{\text{foo}^2}[][]
% defines:
% \foosq{x} -> \text{foo}^2 \left[ x \right]
% \foosq[a]{x} -> \text{foo}^2_a \left[ x \right]
% \foosq[a][\big]{x} -> \text{foo}^2_a \big[ x \big]
% \foosq[][\big]{x} -> \text{foo}^2 \big[ x \big]
% \foosq[][][()]{x} -> \text{foo}^2 \left ( x \right )
% Note that _{} would normally add undesirable space that this definition avoids
\def\OptSubscript#1{\ifthenelse{\equal{#1}{}}{}{_{#1}}}
\def\DeclareOptSubscriptFunction#1#2[#3]#4#5{
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar[{\csname#1@\endcsname}{\csname#1@@@\endcsname[#3][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@\endcsname[##1]{%
    \@ifnextchar[{\csname#1@@\endcsname[##1]}{\csname#1@@@\endcsname[##1][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@@\endcsname[##1][##2]{%
    \@ifnextchar[{\csname#1@@@\endcsname[##1][##2]}{\csname#1@@@\endcsname[##1][##2][{#4}{#5}]}}
  %
   \expandafter\def\csname#1@@@\endcsname[##1][##2][##3##4]##5{%
%               {\ensuremath{#2\OptSubscript{##1}|##2|##3|##4|##5|}}}
               {\ensuremath{#2\OptSubscript{##1}\lr[##2]{##3}{##4}{##5}}}}
}
\def\DeclareOptSubscriptOptArgFunction#1#2[#3]#4#5{
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar[{\csname#1@\endcsname}{\csname#1@@@\endcsname[#3][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@\endcsname[##1]{%
    \@ifnextchar[{\csname#1@@\endcsname[##1]}{\csname#1@@@\endcsname[##1][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@@\endcsname[##1][##2]{%
    \@ifnextchar[{\csname#1@@@\endcsname[##1][##2]}{\csname#1@@@\endcsname[##1][##2][{#4}{#5}]}}
  %
   \expandafter\def\csname#1@@@\endcsname[##1][##2][##3##4]##5{%
     \ifthenelse{\equal{##5{}}{{}}}% if arg is empty omit delimeters
                {\ensuremath{#2\OptSubscript{##1}}}%
                {\ensuremath{#2\OptSubscript{##1}\lr[##2]{##3}{##4}{##5}}}}
}

\makeatother


% probability distributions
\DeclareOptSubscriptOptArgFunction{pr}{{\bf\sf{P}}}[]()
% \DeclareOptSubscriptFunction{prf}{\bf\sf{P}}[]{}{}

% \newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
% \newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
% \newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}

% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\size]{x} -> \mathbb{E}_a \size[ x \size]
\DeclareOptSubscriptFunction{expect}{\mathbb{E}}[][]
\DeclareOptSubscriptFunction{var}{\mathbb{V}}[][]
\DeclareResizableDelimFunction{angles}{}\langle\rangle

% likelihoods
\DeclareOptSubscriptFunction{like}{\mathcal{L}}[]()
\DeclareOptSubscriptFunction{loglike}{\ell}[]()

% info theoretic
\DeclareResizableDelimFunction{entropy}{\textbf{\textsf{H}}}[]
\DeclareResizableDelimFunctionOnTwoArgs{info}{\textbf{\textsf{I}}}[]{\,;}
\def\mutualinfo[#1;#2]{\info{#1}{#2}} % older form
\DeclareResizableDelimFunctionOnTwoArgs{KL}{\textbf{\textsf{KL}}}[]{\lrmid\|}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\DeclareResizableDelimFunctionOnTwoArgs{normal}{\mathcal{N}}(){,}

% whitened quantities
% \newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}
% explicitly defined in some old versions
% \newcommand{\setV}{\ensuremath{{\cal V}}}
% \newcommand{\setX}{\ensuremath{{\cal X}}}
% \newcommand{\setY}{\ensuremath{{\cal Y}}}
% \newcommand{\setZ}{\ensuremath{{\cal Z}}}
\DeclareResizableDelimFunction{size}{}\vert\vert

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\DeclareResizableDelimFunction{norm}{}\|\|
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\let\det\undefined % lose std definition
\DeclareResizableDelimFunction{det}{}\vert\vert
\DeclareResizableDelimFunction{trace}{\mathsf{Tr}}[]
\DeclareResizableDelimFunction{diag}{\mathbox{\textsf{diag}}}[]

% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\makeatletter
\newcommand{\@dx}[1][dx]{%
  \mathchoice{\mkern-3mu}{}{}{}% extra backkern in display
  \mkern-3mu#1\,% 
}
\newcommand{\intdx}[1][dx]{\int\@dx[#1]}

% \mltint -> \int\dots\int with better spacing
% \mltint[3] -> \int\int\int with better spacing
% more compact than amsmath \iint \iiint \idotsint 
\newcounter{multintctr}
\newcommand{\mltint}[1][]{%
  \ifthenelse{\equal{#1{}}{{}}}
    {\int\mkern-6mu{\cdot} %{} kills default space around \cdot
      \mathchoice%
        {\mkern1mu{\cdot}\mkern1mu}% display
        {{\cdot}}% inline
        {{\cdot}}% script
        {{\cdot}}% sscript
      {\cdot}\mkern-6mu}
    {\setcounter{multintctr}{1}%
      \whiledo{\value{multintctr}<#1}{%
        \int\mkern-12mu%
        \stepcounter{multintctr}%
      }}%
    \int}

\def\mltintdx{%
  \@ifnextchar[{\@mltintdx}{\@mltintdx[]}%
}
\def\@mltintdx[#1]{\mltint[#1]\@dx}

\makeatother

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturalss}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}




% accents

% from symbols-a4.pdf; optional arg permits shortening to prevent
% adjacent bars running together
\newcommand{\widebar}[2][3]{{}\mkern#1mu\overline{\mkern-#1mu#2}}

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}

%% overrideable left-right delimeters
% \lr(){foo} -> \left(foo\right)
% \lr[]{foo} -> \left[foo\right]
% \lr[\big](){foo} -> \big({foo}\big)
% \lr[][]{foo} -> \left[{foo}\right]  -- double [] to avoid delims begin processed as (empty) opt
% \lr\{\}{a \lrmid | b } will re-scale the `|' appropriately
% \lr{}{}{foo} -> foo -- this is useful to clobber delims when lr is called from other macros
% this version should nest correctly.  
\newcommand\lr[4][]{%
  \ifthenelse{\equal{#2{}}{{}} \and \equal{#3{}}{{}}}%
             {#4}%
             {\ifthenelse{\equal{#1{}}{{}}}%
               {{\left#2\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
               {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
             }%
}
% \makeatletter
% \newcommand\lr[4][]{%
%   \ifthenelse{\equal{#1{}}{{}}}%
%              {\def\@lrcontent{#4}%
%                \mathopen{\left#2\vphantom\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
%              {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
% }
% \makeatother

% % old version -- use \lrset( \lrset) in place of \left( right).  Cannot be nested!!
% \newboolean{inlr}
% \newboolean{midlr}
% \setboolean{inlr}{false}
% \newcommand\newlr{\setboolean{inlr}{false}}
% 
% \newcommand\lrset[1]{%
%   \ifthenelse{\boolean{inlr}}%
%     {\ifthenelse{\boolean{midlr}}%
%       {\middle#1\setboolean{inlr}{true}}
%       {\right#1}}%
%     {\left#1\setboolean{inlr}{true}}}%
% \newcommand\lrmid{%
%   \ifthenelse{\boolean{inlr}}%
%     {\setboolean{midlr}{true}}
%     {}}%




